The clustering of galaxies in the completed SDSS-III Baryon Oscillation Spectroscopic Survey: theoretical systematics and Baryon Acoustic Oscillations in the galaxy correlation function

We investigate the potential sources of theoretical systematics in the anisotropic Baryon Acoustic Oscillation (BAO) distance scale measurements from the clustering of galaxies in configuration space using the final Data Release (DR12) of the Baryon Oscillation Spectroscopic Survey (BOSS). We perform a detailed study of the impact on BAO measurements from choices in the methodology such as fiducial cosmology, clustering estimators, random catalogues, fitting templates, and covariance matrices. The theoretical systematic uncertainties in BAO parameters are found to be 0.002 in the isotropic dilation $\alpha$ and 0.003 in the quadrupolar dilation $\epsilon$. The leading source of systematic uncertainty is related to the reconstruction techniques. Theoretical uncertainties are sub-dominant compared with the statistical uncertainties for BOSS survey, accounting $0.2\sigma_{stat}$ for $\alpha$ and $0.25\sigma_{stat}$ for $\epsilon$ ($\sigma_{\alpha,stat} \sim$0.010 and $\sigma_{\epsilon,stat}\sim$ 0.012 respectively). We also present BAO-only distance scale constraints from the anisotropic analysis of the correlation function. Our constraints on the angular diameter distance $D_A(z)$ and the Hubble parameter $H(z)$, including both statistical and theoretical systematic uncertainties, are 1.5\% and 2.8\% at $z_{\rm eff}=0.38$, 1.4\% and 2.4\% at $z_{\rm eff}=0.51$, and 1.7\% and 2.6\% at $z_{\rm eff}=0.61$. This paper is part of a set that analyzes the final galaxy clustering dataset from BOSS. The measurements and likelihoods presented here are cross-checked with other BAO analysis in \citet{Acacia16}. The systematic error budget concerning the methodology on post-reconstruction BAO analysis presented here is used in \citet{Acacia16} to produce the final cosmological constraints from BOSS.

==> WedgesErr.tex <==
In order to find the source of this differences in the error distributions we compare the $\chi^2$ surfaces of multipoles and wedges at the mock-by-mock level as a sanity check to guarantee that we are observing a real effect. Figure~.\ref{fig:chi2pae} top panels show the likelihood surfaces of the first mock of the lower redshift bin. The correspondent 1-d distributions are plotted in bottom panels%Figure~.\ref{fig:chi2pae} bottom panels
%: $p(\alpha)$ on the left and $p(\epsilon)$ on the right. $\Delta \chi^2(a)$ and $\Delta \chi^2 (\epsilon)$ are also provided.% in top panels.
% The plots indicate the larger uncertainties are coming from the wider $\chi^2$ surfaces that generates wider $p(\epsilon)$ distributions when marginalising over $\alpha$.  
\begin{figure}
   \centering     
%    \includegraphics[width=1.5in]{mgrid0001_rec.pdf}
%    \includegraphics[width=1.5in]{mgrid0001_rec_wed.pdf}
%   \caption{ $\chi^2(\alpha, \epsilon)$ for different clustering estimators $\xi_{0, 2}$ (left panel?) and $\xi_{\parallel, \perp}$ (right panel?) for a single MD-PATCHY post-reconstruction mock for the lowest redshift bin. \comment{why not fit the mean of the mocks?}%\comment{could this be combined with current fig4?} }
%   \label{fig:chi2ae}
%\end{figure}
%
%\begin{figure}
%   \centering     
    \includegraphics[width=3.5in]{chi_rec.pdf}
    \includegraphics[width=3.5in]{chi_rec_wed.pdf}
   \caption{ %Top panel. $\chi^2(\alpha, \epsilon)$ for different clustering estimators $\xi_{0, 2}$ (left panel?) and $\xi_{\parallel, \perp}$ (right panel?) for a single MD-PATCHY post-reconstruction mock for the lowest redshift bin. %\comment{why not fit the mean of the mocks?}
   Bottom panel. $\Delta \chi^2(\alpha)$ (top left), $\Delta \chi^2 (\epsilon)$ (top right), $p(\alpha)$ (bottom left) and $p(\epsilon)$ (bottom right) for different clustering estimators $\xi_{0, 2}$ (top four plots) and $\xi_{\parallel, \perp}$ (bottom four plots) for 1 MD-PATCHY post-reconstruction mock for the lowest redshift bin. \commentH{not sure if these plots are useful for this explanation but my goal was to show this effect is real and not a bug in the fitting code, suggestions? } \commentH{why not fit the mean of the mocks?}}
   \label{fig:chi2pae}
\end{figure}

==> data_DR12.tex <==
In previous sections, we present a detailed investigation of possible sources of theoretical systematics in anisotropic BAO measurements. We have applied all the variants of the methodology to mock observations as described in Sec~\ref{main_sys}, and investigated the expected precision and systematics for our methodology. 

We will now apply our methodology as described in section~\ref{method} to our BOSS dataset. We use the final BOSS combined catalog from Data Release 12 of Sloan Digital Sky Survey, as described in Sec~\ref{sec:data}. 
We  apply all weights described in \ref{Ross16} which included weights related to seeing, stellar densities, fiber collisions, redshift failures and a weight to optimize the power of the clustering for BAO measurements (FKP weights). 
Now, we first calculate the pair-counts for the catalogs, and then compute various clustering estimators before reconstruction for the sample as seen in Figure~\ref{figXX} for multipoles, Figure~\ref{figXX} for Wedges and Figure~\ref{figXX}  for $\omega_l$ clustering estimator. 
We then apply our reconstruction algorithms onto our data, and show the different resulting clustering estimators for the data in Figure \ref{fig:datamultipole},\ref{fig:datawed} and \ref{fig:dataomega} for all three redshift bins in the catalog. 
The error bars are given by the diagonal terms of the covariance matrix computed from the MD-PATCHY mock catalogs. 
The post-reconstruction results show the expected sharpening of BAO peaks as well as  the decrease in the amplitude due to the corrections for redshift space distortions. 

The lower redshift bin seems to be systematically higher amplitude post-reconstruction and also it seems to differ more from the mean of PATCHY mocks. The new feature of this multipoles presentation is the hexadecapole contribution, that is very small and with twice large error bars compared with quadrupole. 

The wedges, ($\xi_{||,\perp}$) are shown in Figure \ref{fig:datawed}. we observe the sharpening of the peak and the decrease in amplitude of the wedges post-reconstruction. \comment{comment the Figure. Maybe change the mean of the mocks for the best fit?}

In  Figure \ref{fig:dataomega} we show the $\omega_l$ estimator. Wedges follow the same trend as multipoles for the lower redshift bin that is systematically higher compared to the other redshift bins.

\begin{figure}
   \centering     
     \includegraphics[width=3.3in]{Hexadecapole-post_data.pdf}
   \caption{\comment{Shirley rewrote the caption, since it looks like this is DATA instead of mean of 1000 mocks} 
  We present the multipoles of the final BOSS combined sample post-reconstruction in three redshift bins. }
% Multipoles Clustering Estimator: Mean of  mocks pre-reconstruction [left] and post-reconstruction [right] for 1000 MD-PATCHY for the 3 redshift bins.}
   \label{fig:datamultipole}
\end{figure}

\begin{figure}
   \centering     
    \includegraphics[width=3.5in]{Wedges-DR12-post.pdf}
   \caption{\comment{shirley rewrote this caption, since it looks like DR12} We present the clustering wedges of the final BOSS combined sample post-reconstruction in three redshift bins.}
   \label{fig:datawed}
\end{figure}

\begin{figure}
   \centering     
    \includegraphics[width=3.5in]{Omega-DR12-post.pdf}
   \caption{ We present the $\omega_l$ clustering statistics for final BOSS combined sample post-reconstruction in three redshift bins.}
   %\caption{ $\omega_l$ Clustering Estimators: Mean of  mocks pre-reconstruction [left] and post-reconstruction [right] for 1000 MD-PATCHY for the 3 redshift bins.}
   \label{fig:dataomega}
\end{figure}
The results for applying the anisotropic methodology to the COMBINED samples of BOSS are presented in Tables \ref{tab:fitsdr12a} and \ref{tab:fitsdr12b} considering the different variants of the methodology explored in the paper. We focus here in the differences in $\alpha$ and $\epsilon$ and their uncertainties and we are going to compare with the dispersions we get from the mocks to be able to judge any significant deviation.\comment{Analyze results presented in the table, highlight the differences or similarities in alpha and epsilon and their uncertainties.}

\comment{Dispersion plot to be included to show how correlated are the BAO measurements between estimators and how this compares with the results in this section are the differences observed in the data BAO parameters consistent with results obtained on the mocks?}
\begin{figure*}
   \centering     
     \includegraphics[width=5.3in]{Covariance_data_plots.pdf}%\includegraphics[width=2.3in]{Modelcov_data_plot.pdf}
   \caption{ Comparison of errors in $\alpha$ and $\epsilon$ between mocks and data for lower redshift bin. Left, using the covariance from QPM, right using the covariance from Patchy}%, on the right using the model covariance \comment{Model is using only 300 mocks}.}
   \label{fig:dataHexa}
\end{figure*}
\begin{figure*}
   \centering     
     \includegraphics[width=6.3in]{Estimators_data_plot.pdf}
   \caption{ Comparison of errors in $\alpha$ and $\epsilon$ between mocks and data for lower redshift bin. Left, using multipoles, center using $\omega$ and right using wedges.}%, on the right using the model covariance \comment{Model is using only 300 mocks}.}
   \label{fig:dataHexa}
\end{figure*}


\begin{figure}
   \centering     
     \includegraphics[width=3.3in]{ALpha_comp.pdf}
     \includegraphics[width=3.3in]{Epsilon_comp.pdf}
   \caption{ Fits and Errors from fitting lower redshift bin of BOSS data. Left, $\alpha$ and $\sigma\alpha$ from fitting using a variant in the BAO methodology. [Right] $\epsilon$ and $\sigma_\epsilon$, the dotted lines are the mean of the different measurements, the dotted lines are the difference of mean by 0.2\% and 0.5\%. in $\alpha$ and $\epsilon$ respectively.}
   \label{fig:dataHexa}
\end{figure}
%\rr{Shirley: table commented out due to compilation issues} 
%commented out to see whether the files will compile
\input{table_data_diff_post}







==> randomtest_old.tex <==
The computation of 2-point estimators requires the generation of a random set matching the survey geometry and completeness. The error on the correlation function due to the  number of randoms is related to the error in the determination of the correlation function for a given sample. In the limit of an infinite random set, the noise contribution from the randoms  is zero. However, in practise using a large number of randoms significantly increases  the cost of computing the estimator in the analysis.  In this section, we test the effect of using different sizes of the random catalogue in anisotropic fits.

For the pre-reconstruction case, the RR and RD pair-counts used in the Landy-Szalay estimator are computed once for all the mocks. The finite size of the randoms coupled with the fact that we use the same random file for all of the mocks is a potential source of scatter that is not in the covariance matrix. We test using two different sets of randoms. If we use a single random catalogue, we might get some small shift that is purely from that random catalogue not being infinite. The difference between that shift and the shift found from a much larger random catalogue should indeed tell you something about the size of the systematic uncertainty.

For the post-reconstruction case the approach is slightly different.  In the post-reconstruction case, there are two sets of random catalogues: the denominator randoms used to determine the geometry of the survey, and the numerator randoms that we shift according to the displacement field inferred from data; we call this, shifted random catalogue. The shifted random catalogue is  different for every single mock, thus the DS and SS counts need to be recomputed for each mock. %Thus the computational cost of the randoms is dramatically increased compared to the pre-reconstruction case where the RR pair-counts are computed once for all the mocks.
 From the definition of the Landy-Szalay estimator, we know that the variance in the correlation functions is dominated by the DR paircounts, which goes to as $4/x$ (where $x$ is the ratio of randoms-to-data), with the RR paircounts being subdominant, scaling as $1/x^2$. Thus, if we use $x=4$ the variance is 10 times bigger than if we use $x=40$. Thus, we decided to test the effect of the the size of the random catalogues in this case for the $SS$ term for balancing the errors in the correlation function estimate. \footnote{In particular, computing the post-reconstruction correlation function requires the computation of very expensive random-random pair-counts for each one of our thousands of mocks catalogues. Thus, this tests is critical for minimizing the computational cost of  doing so for 1000 post-reconstruction mocks for the 3 redshift bins.}





\subsection{Random size Pre-reconstruction}

 We test the effect of the randoms pre-reconstruction with 100 QPM CMASS mocks; we use as fiducial cosmology, the natural cosmology of the QPM mocks (see Table~\ref{tab:cosmofid}).
We test two random sets: the first case is a random set 20 times the size of the data sample, denoted by ``$20x$", and a second set 50 times the size of the data sample, denoted by ``$50x$". We computed the multipoles using these two set of randoms and then 
we performed anisotropic analysis described in Section~\ref{sec:method}.  
The results are shown in Table~\ref{tab:randtest_delta}; we report the mean difference of fits performed on the correlation functions using $20x$ compared to the correlation functions computed with $50x$ randoms.

\begin{table}
\begin{center}
\caption{Fitting results from QPM CMASS mocks Pre/Post-Reconstruction: Random Test (Section~\ref{sec:randoms}). The variations in the best fits are defined as: $\Delta \alpha=\alpha_{50x}-\alpha_{20x}$ and $\Delta \epsilon=\epsilon_{50x}-\epsilon_{20x}$ for pre-reconstruction test.
$\Delta \alpha=\alpha_{50x}-\alpha_{4x}$ and $\Delta \epsilon=\epsilon_{50x}-\epsilon_{4x}$ for post-reconstruction test.}% \comment{Check numbers again for randoms and propagate}}
\label{tab:randtest_delta}
\begin{tabular}{@{}lcc} 
\hline
Set&$|<\Delta \alpha>| \pm$ RMS & $|<\Delta \epsilon>| \pm$ RMS \\
\hline
CMASS Pre-Rec&0.0008 $\pm$ 0.0038&0.0006 $\pm$ 0.0066 \\
\hline
Bin 1 Post-Rec&0.0002 $\pm$ 0.0017&0.0003 $\pm$ 0.0035\\
\\[-1.5ex]
Bin 2 Post-Rec&0.0002 $\pm$ 0.0011&$<$0.0001 $\pm$ 0.0015\\
\\[-1.5ex]
Bin 3 Post-Rec& 0.0001 $\pm$ 0.0015&$<$0.0001 $\pm$ 0.0017\\
\hline
RMS &0.0002&0.0002\\
\hline
\end{tabular}
\end{center}
\end{table}

The main conclusion is that randoms make very small differences in the mean of isotropic/anisotropic fits for both of these two cases. The differences observed are $\le 0.0002$. 

\subsection{Different number of randoms for DR and RR terms post-reconstruction}
 We test the effect of the randoms post-reconstruction with 100 QPM CMASS mocks; we use as fiducial cosmology, the natural cosmology of the QPM mocks (see Table~\ref{tab:cosmofid}). We test the effect of randoms differently that pre-reconstruction. We reduce the number of randoms from $50x$ to $4x$  for post-reconstruction correlation functions in the numerator  SS (not for the SR term)  and we test the impact on the fitting parameters. 
%We study the effect  of randoms for the pre/post-reconstruction pair-counts. 
%AS:For the random test, I would have thought we would want to know if the standard deviation changes at all. Naively, I would think that the fits should be unbiased, but one might expect more noise if there are less randoms. If you have the numbers on the standard deviations, it might be good to show those...
% In Figure~\ref{fig:difant} we show the test performed with 100 mocks between $50x$ and $4x$.
% Differences between the $50x$ and the $4x$ correlation functions are 1-2$\sigma$ (defined as the RMS of the $50x$ mocks at each radial bin)  
% at the BAO scale, and up to $3\sigma$ at the largest scales used in the fitting, in particular for Bin 3.  The differences between the correlation functions might be minimized by running several SS $4x$ counts and averaging them. However, using different sizes of random catalogues for SS and DS counts would still save us a lot of computing time as compared to the $50x$ case. 
%We conclude that in order to get less than $1\sigma$ differences between the correlation function with the sub-sampled set of randoms and the same correlation function using the full ($50x$) set of randoms, $4x$ is not enough (Figure \ref{fig:difant} Rows 1-2). %But we do not need to go to $20x$ either (Figure \ref{fig:difant} Rows 3-4).
%  An interesting feature in the plots in Figure \ref{fig:difant} is that the quadrupoles (bottom panels) fluctuate  less than the monopoles (top panels), which is related to the values found in the anisotropic fits (Table~\ref{tab:randtest_delta}).
%We now move on to the variations in the anisotropic fits.
We show the results in table \ref{tab:randtest_delta} ( Table \ref{tab:randtest} in the appendix show the results of the best fits distributions obtained  with100 mock catalogues.
% We show in table \ref{tab:randtest} the mean/RMS of 100 mock results. %We quoted and also the difference in fitted parameters. 
 %As we are interested only in 
 The differences between the $50x$ and the $4x$ anisotropic fits are very small: $0.0002$ for $\alpha$ and $0.0002$ for $\epsilon$. 
%In principle, 
The variations in the anisotropic fits when using different numbers of randoms must be random (i.e., not systematic); these variations must be statistical fluctuations and they should be in our covariance matrices if we use the same numbers of randoms. However, the finite size of the randoms is a potential source of scatter that is not in the covariance matrix, and what are demonstrating is that %this potential source of scatter 
it is not contributing significantly to the scatter. %If we use a single random catalogue, we might get some small shift that is purely from that random catalogue not being infinite. The difference between that shift and the shift found from a much larger random catalogue should indeed tell you something about the size of the systematic uncertainty. We summarize the differences find in Table~\ref{tab:randtest_delta} to assess the size of the potential systematic uncertainty. 
%As expected, the random size is not causing any significant shift on the BAO feature, however it can add to the noise in the location of the BAO peak, hence increasing the uncertainty of distance scale measurement.

 %we extrapolate the results of the scatter observed in the cases analyzed ($4x$, $20x$ and $50x$) to the $100x$ randoms (Figure \ref{ExtrapRand}). The results for the standard deviation are shown in the \ref{tab:randtest}. For obtaining the $\Delta \sigma_{\alpha, \epsilon}$ we defined our fiducial case as the $50x$ randoms used for the data and we estimate the difference with the $100x$. The variations in the scatter are very small ($<$0.0001). 
%
%\begin{figure}
%\includegraphics[width=1.in]{diff_4x_50x_bin1_monopole.png}
%\includegraphics[width=1.in]{diff_4x_50x_bin2_monopole.png}
%  \includegraphics[width=1.in]{diff_4x_50x_bin3_monopole.png}
% \includegraphics[width=1.in]{diff_4x_50x_bin1_quadrupole.png} 
%   \includegraphics[width=1.in]{diff_4x_50x_bin2_quadrupole.png}
%    \includegraphics[width=1.in]{diff_4x_50x_bin3_quadrupole.png}         
%% \includegraphics[width=1.in]{diff_20x_50x_bin1_monopole.png}
%% \includegraphics[width=1.in]{diff_20x_50x_bin2_monopole.png}
%%     \includegraphics[width=1.in]{diff_20x_50x_bin3_monopole.png}
%% \includegraphics[width=1.05in]{diff_20x_50x_bin1_monopole.png}
%% \includegraphics[width=1.05in]{diff_20x_50x_bin2_quadrupole.png}
%% \includegraphics[width=1.05in]{diff_20x_50x_bin3_quadrupole.png}
%   \caption{Difference between the correlation function computed with 50x randoms in the (post-reconstruction) random-random paircounts, and the correlation function (for the same mock) computed with 4x (first 2 rows of plots) %and $20x$ randoms (rows 3-4 of plots) 
%   for the monopole (top) and the quadrupole (bottom). The differences are normalised by the RMS of the $50x$ mocks at each radial bin. For each row, the left panel shows the correlation functions in redshift bin $0.20<z<0.50$, middle panel corresponds to redshift bin $0.40<z<0.60$, and right panel represents the redshift bin $0.50<z<0.75$.}
%   \label{fig:difant}
%\end{figure}





As an additional output of this test, the results validate the use $50x$ pair-counts for DS pair-counts and $7x$ for SS for the mock covariance  for \cite{Acacia16}. With the current 2-point correlation code [Reference to Padmanabhan code]  and the number of mocks required for doing BAO/RSD analysis using the correlation function, a total of 132,000 CPU-hours were required for estimating the post-reconstruction pair counts using EDISON at NERSC. DR12 correlation functions were computed with $50x$ randoms pre and post-reconstruction.
  
We conclude that there is no systematic error in BAO distance measurements associated to the number of randoms. % is $0.0002$ for $\alpha$ and $0.0002$\  for $\epsilon$. 
The variations in the scatter are $<0.0001$ in $\alpha$ and $\epsilon$. %}.
 
 
% We conclude that the systematic error in BAO distance measurements associated to the number of randoms is $0.0002$ for $\alpha$ and $0.0002$\  for $\epsilon$. 


==> table_data_diff_postonly.tex <==
\begin{table*}  
\caption{Fitting results from Combined DR12 samples in the three redshift bins. $\Delta x$ is the difference with respect to the fiducial case (first row)}
\label{tab:fitsdr12a}

\begin{tabular}{@{}lcccccccc}
\hline
\multicolumn{8}{c}{Testing Variants of Methodology on DR12}\\
\hline
\multicolumn{8}{c}{DR12 Combined Samples Post-reconstruction}\\
\hline
\multicolumn{8}{c}{BIN 1 ($0.2 < z < 0.5$)}\\
\hline

Variable&$\alpha \pm \sigma_\alpha$ & $\Delta \alpha$&$\Delta \sigma_\alpha$&$\epsilon \pm \sigma_\epsilon$ &$\Delta \epsilon$&$\Delta \sigma_\epsilon$&$ \chi^2$ \\%&
%$\alpha_{||} \pm \sigma_{\alpha_{||}}$& $\alpha_{\perp} \pm \sigma_{\alpha_{\perp}}$\\
\hline

PAT cov &
$0.9995\pm 0.0098$&-&-&$0.0152 \pm 0.0125$&&&$40.8881$\\%&
%$1.0301 \pm 0.0284$&$0.9845 \pm 0.0145$\\
\hline
QPM cov &
$0.9976\pm 0.0091$& -0.0019& -0.0007&$0.0159\pm 0.0119$&0.0007&-0.0006&$1.5467$\\%&
%$1.0296\pm 0.0277$&$0.9819\pm 0.0129$\\
\\[-1.5ex]

Model Cov&
$0.9971\pm 0.0090$& -0.0023& -0.0008&$0.0113\pm 0.0118$&-0.0039&-0.0006&$1.3726$\\%&
%$1.0199\pm 0.0274$&$0.9859\pm 0.0129$\\
\hline
$\xi_{\parallel, \perp}$ &
%$0.9982\pm 0.0103$& -0.0013& 0.0005&$-0.0136\pm 0.0154$&-0.0288&0.0029&$1.1784$\\%&
%$0.9713\pm 0.0316$&$1.0119\pm 0.0191$\\
$0.9986\pm 0.0103$& -0.0009& 0.0005&$0.0153\pm 0.0154$&0.0001&0.0029&$1.1616$\\%&
%$1.0294\pm 0.0326$&$0.9835\pm 0.0182$\\

\\[-1.5ex]

$\xi_{l=4}$&
$1.0002\pm 0.0097$& 0.0008& -0.0001&$0.0097\pm 0.0102$&-0.0055&-0.0022&$1.9752$\\%&
%$1.0198\pm 0.0237$&$0.9906\pm 0.0133$\\

\\[-1.5ex]

$\omega_l$ &
$0.9962\pm 0.0113$& -0.0033& 0.0015&$-0.0003\pm 0.0145$&-0.0155&0.0021&$0.1221$\\%&
%$0.9956\pm 0.0324$&$0.9964\pm 0.0172$\\
\hline
%$C_{MG,30}$&
%$0.9964\pm 0.0095$& -0.0030& -0.0003&$0.0109\pm 0.0099$&-0.0043&-0.0026&$1.9560$\\%&
%$1.0183\pm 0.0228$&$0.9857\pm 0.0130$\\
%\\[-1.5ex]

$C_{MG,60}$&
$0.9993\pm 0.0099$& -0.0002& 0.0000&$0.0140\pm 0.0127$&-0.0012&0.0002&$1.3633$\\%&
%$1.0275\pm 0.0293$&$0.9854\pm 0.0142$\\
%\\[-1.5ex]
%
%$C_{G,30}$&
%$0.9989\pm 0.0098$& -0.0006& -0.0000&$0.0153\pm 0.0126$&0.0001&0.0002&$2.1771$&
%$1.0297\pm 0.0282$&$0.9839\pm 0.0151$\\
\hline
%\multicolumn{8}{c}{DR12 Combined Samples Pre-reconstruction}\\
%\hline
%PAT&$1.0037\pm 0.0147$& -& -&$0.0241\pm 0.0168$&-&-&$1.2838$\\%&
%%$1.0525\pm 0.0392$&$0.9801\pm 0.0206$\\
%\hline
%QPM cov&
%$1.0073\pm 0.0135$& 0.0036& -0.0012&$0.0260\pm 0.0154$&0.0019&-0.0014&$1.4904$\\%&
%%$1.0603\pm 0.0369$&$0.9818\pm 0.0182$\\
%\\[-1.5ex]
%%Model cov&\\
%\hline
%$\xi_{\parallel, \perp}$&
%$1.0068\pm 0.0195$& 0.0031& 0.0048&$-0.0228\pm 0.0154$&-0.0468&-0.0015&$1.3305$\\%&
%%$0.9615\pm 0.0351$&$1.0302\pm 0.0260$\\
%\\[-1.5ex]
%$\xi_{l=4}$&
%$1.0027\pm 0.0097$& -0.0010& -0.0050&$0.0095\pm 0.0102$&-0.0146&-0.0066&$1.9999$\\%&
%%$1.0218\pm 0.0237$&$0.9933\pm 0.0134$\\
%\\[-1.5ex]
%$\omega_l$ &
%$1.0026\pm 0.0148$& -0.0010& 0.0001&$0.0114\pm 0.0204$&-0.0126&0.0035&$1.5093$\\%&
%%$1.0257\pm 0.0503$&$0.9913\pm 0.0183$\\
%\\[-1.5ex]

%\hline
\end{tabular}
\end{table*}


\begin{table*}  
\caption{Fitting results from Combined DR12 samples in the intermediate redshift bin. $\Delta x$ is the difference with respect to the fiducial case  (first row).\commentH{what does +1, +2, +3, +4 mean?} }\label{tab:fitsdr12b}
\begin{tabular}{@{}lcccccccc}
\hline
\multicolumn{8}{c}{Testing Variants of Methodology on DR12}\\
\hline
\multicolumn{8}{c}{DR12 Combined Samples Post-reconstruction}\\
\hline
\multicolumn{8}{c}{BIN 2 ($0.4 < z < 0.6$)}\\
\hline
Variable&$\alpha \pm \sigma_\alpha$ & $\Delta \alpha$&$\Delta \sigma_\alpha$&$\epsilon \pm \sigma_\epsilon$ &$\Delta \epsilon$&$\Delta \sigma_\epsilon$&$ \chi^2$ \\%&
%$\alpha_{||} \pm \sigma_{\alpha_{||}}$& $\alpha_{\perp} \pm \sigma_{\alpha_{\perp}}$\\
\hline
PAT&
$0.9928\pm 0.0084$&-&-&$-0.0036 \pm 0.0107$&-&-&$19.0635$\\%&
%$0.9856 \pm 0.0227$&$0.9964 \pm 0.0136$\\
\hline
QPM cov&
$0.9929\pm 0.0080$& 0.0001& -0.0004&$-0.0016\pm 0.0103$&0.0021&-0.0004&$0.6913$\\%&
%$0.9897\pm 0.0221$&$0.9944\pm 0.0128$\\
\\[-1.5ex]
Model cov&
$0.9923\pm 0.0078$& -0.0005& -0.0006&$-0.0035\pm 0.0106$&0.0002&-0.0001&$0.6808$\\%&
%$0.9854\pm 0.0228$&$0.9957\pm 0.0127$\\
\hline
$\xi_{\parallel \perp}$&
%$0.9916\pm 0.0089$& -0.0012& 0.0005&$0.0012\pm 0.0140$&0.0048&0.0034&$0.6553$\\%&
%$0.9940\pm 0.0303$&$0.9904\pm 0.0155$\\
$0.9917\pm 0.0089$& -0.0010& 0.0005&$-0.0008\pm 0.0140$&0.0029&0.0034&$0.6572$\\%&
%$0.9902\pm 0.0303$&$0.9925\pm 0.0155$\\
\\[-1.5ex]
$\xi_{l=4}$&
$0.9968\pm 0.0088$& 0.0040& 0.0004&$-0.0032\pm 0.0099$&0.0005&-0.0008&$3.7024$\\%&
%$0.9906\pm 0.0216$&$1.0000\pm 0.0131$\\
\\[-1.5ex]
$\omega_l$&
$0.9994\pm 0.0104$& 0.0066& 0.0020&$0.0035\pm 0.0129$&0.0072&0.0022&$0.1182$\\%&
%$1.0065\pm 0.0295$&$0.9959\pm 0.0150$\\
\hline
$C_{MG 60}$&
$0.9924\pm 0.0083$& -0.0004& -0.0001&$-0.0037\pm 0.0100$&-0.0001&-0.0007&$0.6213$\\%&
%$0.9851\pm 0.0216$&$0.9961\pm 0.0128$\\
%\\[-1.5ex]
%$C_{G30}$&
%$0.9939\pm 0.0082$& 0.0011& -0.0002&$-0.0035\pm 0.0106$&0.0001&-0.0000&$0.9811$\\%&
%%$0.9869\pm 0.0226$&$0.9974\pm 0.0134$\\
%\hline
%$+1$&
%$0.9947\pm 0.0048$& 0.0019& -0.0036&$-0.0031\pm 0.0040$&0.0005&-0.0066&$1.7668$&
%$0.9885\pm 0.0096$&$0.9978\pm 0.0061$\\
%\\[-1.5ex]
%$+2 $&
%$0.9937\pm 0.0051$& 0.0009& -0.0033&$-0.0028\pm 0.0042$&0.0008&-0.0065&$2.9671$&
%$0.9882\pm 0.0104$&$0.9965\pm 0.0061$\\
%\\[-1.5ex]
%$+3$&
%$0.9953\pm 0.0049$& 0.0025& -0.0035&$-0.0020\pm 0.0041$&0.0017&-0.0066&$2.6796$&
%$0.9914\pm 0.0099$&$0.9973\pm 0.0061$\\
%\\[-1.5ex]
%$+4 $&
%$1.0050\pm 0.0051$& 0.0122& -0.0033&$-0.0021\pm 0.0042$&0.0016&-0.0065&$2.0754$&
%$1.0008\pm 0.0097$&$1.0071\pm 0.0066$\\
%\hline
%$60-120$&
%$0.9890\pm 0.0092$& -0.0038& 0.0008&$-0.0027\pm 0.0129$&0.0009&0.0023&$0.3918$\\%&
%%$0.9836\pm 0.0273$&$0.9917\pm 0.0156$\\
%\\[-1.5ex]
%$60-130$&
%$0.9932\pm 0.0084$& 0.0004& 0.0000&$-0.0041\pm 0.0109$&-0.0005&0.0002&$0.4936$\\%&
%%$0.9850\pm 0.0234$&$0.9973\pm 0.0135$\\
%\\[-1.5ex]
%$60-140 $&
%$0.9934\pm 0.0083$& 0.0007& -0.0001&$-0.0042\pm 0.0108$&-0.0005&0.0001&$0.4943$\\%&
%%$0.9852\pm 0.0232$&$0.9976\pm 0.0134$\\
%\\[-1.5ex]
%$60-150 $&
%$0.9931\pm 0.0084$& 0.0003& 0.0000&$-0.0032\pm 0.0107$&0.0004&0.0000&$0.6002$\\%&
%%$0.9867\pm 0.0228$&$0.9963\pm 0.0136$\\
%\\[-1.5ex]
%$60-160 $&
%$0.9922\pm 0.0086$& -0.0006& 0.0002&$-0.0038\pm 0.0109$&-0.0001&0.0002&$0.8585$\\%&
%%$0.9848\pm 0.0236$&$0.9959\pm 0.0135$\\
%\\[-1.5ex]
%$60-170 $&
%$0.9933\pm 0.0085$& 0.0005& 0.0001&$-0.0033\pm 0.0108$&0.0004&0.0001&$1.0479$\\%&
%%$0.9868\pm 0.0233$&$0.9966\pm 0.0135$\\
%\hline
%$30-155 $&
%$0.9939\pm 0.0082$& 0.0011& -0.0002&$-0.0035\pm 0.0106$&0.0001&-0.0000&$0.9811$\\%&
%%$0.9869\pm 0.0226$&$0.9974\pm 0.0134$\\
%\\[-1.5ex]
%$40-155 $&
%$0.9927\pm 0.0083$& -0.0001& -0.0001&$-0.0033\pm 0.0107$&0.0003&0.0000&$0.7583$\\%&
%%$0.9862\pm 0.0229$&$0.9960\pm 0.0133$\\
%\\[-1.5ex]
%$50-155 $&
%$0.9929\pm 0.0083$& 0.0001& -0.0001&$-0.0034\pm 0.0107$&0.0002&-0.0000&$0.7237$\\%&
%%$0.9861\pm 0.0228$&$0.9964\pm 0.0134$\\
%\\[-1.5ex]
%$70-155 $&
%$0.9923\pm 0.0080$& -0.0005& -0.0004&$-0.0039\pm 0.0094$&-0.0003&-0.0012&$0.5746\\$%&
%%$0.9846\pm 0.0202$&$0.9962\pm 0.0125$\\
%\\[-1.5ex]
%$80-155$&
%$1.0326\pm 0.0433$& 0.0398& 0.0349&$-0.0184\pm 0.0736$&-0.0147&0.0629&$1.2508$\\%&
%$0.9950\pm 0.1795$&$1.0519\pm 0.0610$\\
\hline
%\multicolumn{8}{c}{DR12 Combined Samples Pre-reconstruction}\\
%\hline
%PAT cov &
%$1.0112\pm 0.0210$& -& -&$0.0059\pm 0.0302$&-&-&$1.5637$\\%&
%%$1.0231\pm 0.0771$&$1.0053\pm 0.0229$\\
%\hline
%QPM cov&
%$1.0182\pm 0.0168$& 0.0070& -0.0042&$0.0058\pm 0.0223$&-0.0001&-0.0079&$1.6968$\\%&
%%$1.0299\pm 0.0564$&$1.0124\pm 0.0199$\\
%\\[-1.5ex]
%%Model cov&\\
%\hline
%$\xi_{\parallel \perp}$&
%$1.0146\pm 0.0332$& 0.0035& 0.0123&$-0.0056\pm 0.0246$&-0.0114&-0.0056&$1.6239$\\%&
%%$1.0034\pm 0.0453$&$1.0203\pm 0.0501$\\
%\\[-1.5ex]
%$\xi_{l=4}$&
%$0.9987\pm 0.0127$& -0.0125& -0.0082&$-0.0071\pm 0.0182$&-0.0129&-0.0120&$4.0143$\\%&
%%$0.9846\pm 0.0410$&$1.0058\pm 0.0197$\\
%\\[-1.5ex]
%$\omega_l$&
%$1.0012\pm 0.0151$& -0.0100& -0.0059&$-0.0016\pm 0.0201$&-0.0074&-0.0101&$1.2491$\\%&
%%$0.9981\pm 0.0487$&$1.0028\pm 0.0192$\\
%\hline
\end{tabular}
\end{table*}

\begin{table*}  
\caption{Fitting results from Combined DR12 samples in the high redshift bin. $\Delta x$ is the difference with respect to the fiducial case (first row).} \label{tab:fitsdr12c}
\begin{tabular}{@{}lcccccccc}
\hline
\multicolumn{8}{c}{Testing Variants of Methodology on DR12}\\
\hline
\multicolumn{8}{c}{DR12 Combined Samples Post-reconstruction}\\
\hline
\multicolumn{8}{c}{BIN 3 ($0.5 < z < 0.75$)}\\
\hline
Variable&$\alpha \pm \sigma_\alpha$ & $\Delta \alpha$&$\Delta \sigma_\alpha$&$\epsilon \pm \sigma_\epsilon$ &$\Delta \epsilon$&$\Delta \sigma_\epsilon$&$ \chi^2/d.o.f$ \\%&
%$\alpha_{||} \pm \sigma_{\alpha_{||}}$& $\alpha_{\perp} \pm \sigma_{\alpha_{\perp}}$\\
\hline
PAT cov&
$0.9820\pm 0.0091$&-&-&$-0.0109 \pm 0.0125$&-&-&0.9743 \\%&
%$0.9608 \pm 0.0254$&$0.9928 \pm 0.0160$\\
%\\[-1.5ex]
\hline
QPM cov&
$0.9815\pm 0.0094$& -0.0005& 0.0003&$-0.0102\pm 0.0131$&0.0006&0.0006&$1.0400$\\%&
%$0.9615\pm 0.0279$&$0.9916\pm 0.0154$\\
\\[-1.5ex]
Model cov&
$0.9820\pm 0.0092$& 0.0000& 0.0001&$-0.0109\pm 0.0130$&0.0000&0.0005&$0.9744$\\%&
%$0.9608\pm 0.0273$&$0.9928\pm 0.0156$\\
%\\[-1.5ex]
\hline
$\xi_{\parallel \perp}$&
$0.9816\pm 0.0094$& -0.0004& 0.0003&$0.0131\pm 0.0163$&0.0240&0.0038&$1.0766$\\%&
%$1.0075\pm 0.0355$&$0.9689\pm 0.0167$\\
\\[-1.5ex]
$\xi_{l=4}$&
$0.9821\pm 0.0091$& 0.0001& 0.0000&$-0.0153\pm 0.0127$&-0.0044&0.0001&$1.5922$\\%&
%$0.9523\pm 0.0257$&$0.9973\pm 0.0161$\\
\\[-1.5ex]
$\omega_l$&
$0.9989\pm 0.0105$& 0.0169& 0.0015&$0.0010\pm 0.0135$&0.0119&0.0010&$0.1086$\\%&
%$1.0009\pm 0.0303$&$0.9978\pm 0.0161$\\
%\\[-1.5ex]
\hline
%$C_{MG 30}$&
%$0.9828\pm 0.0086$& 0.0008& -0.0005&$-0.0125\pm 0.0101$&-0.0016&-0.0024&$1.4359$\\%&
%%$0.9584\pm 0.0203$&$0.9952\pm 0.0143$\\
%\\[-1.5ex]
$C_{MG 60}$&
$0.9812\pm 0.0088$& -0.0008& -0.0003&$-0.0116\pm 0.0108$&-0.0007&-0.0017&$1.0026$\\%&
%$0.9586\pm 0.0220$&$0.9927\pm 0.0146$\\
%\\[-1.5ex]
%$C_{G 30}$&
%$0.9836\pm 0.0087$& 0.0016& -0.0004&$-0.0124\pm 0.0123$&-0.0016&-0.0003&$1.6777$\\%&
%%$0.9593\pm 0.0245$&$0.9960\pm 0.0159$\\
\hline
%\multicolumn{8}{c}{DR12 Combined Samples Pre-reconstruction}\\
%\hline
%PAT&
%$0.9859\pm 0.0186$& -& -&$-0.0143\pm 0.0253$&-&-&$1.0008$\\%&
%%$0.9578\pm 0.0587$&$1.0002\pm 0.0251$\\
%\hline
%QPM cov&
%$0.9883\pm 0.0184$& 0.0024& -0.0001&$-0.0088\pm 0.0248$&0.0055&-0.0005&$1.0361$\\%&
%%$0.9709\pm 0.0573$&$0.9971\pm 0.0254$\\
%\\[-1.5ex]
%%Model cov&\\
%\hline
%$\xi_{\parallel \perp}$&
%$0.9822\pm 0.0218$& -0.0037& 0.0033&$0.0069\pm 0.0391$&0.0212&0.0138&$1.1329$\\%&
%%$0.9957\pm 0.0893$&$0.9755\pm 0.0340$\\
%\\[-1.5ex]
%$\xi_{l=4}$&
%$0.9910\pm 0.0130$& 0.0051& -0.0056&$-0.0030\pm 0.0191$&0.0113&-0.0062&$3.0203$\\%&
%%$0.9850\pm 0.0419$&$0.9940\pm 0.0212$\\
%\\[-1.5ex]
%$\omega_l$&
%$0.9894\pm 0.0155$& 0.0035& -0.0031&$-0.0079\pm 0.0210$&0.0064&-0.0043&$1.4573$\\%&
%%$0.9738\pm 0.0491$&$0.9973\pm 0.0209$\\
%\hline
\end{tabular}
\end{table*}

